Monocular 3D Object Detection and Box Fitting Trained End-to-End Using Intersection-over-Union Loss

Three-dimensional object detection from a single view is a challenging task which, if performed with good accuracy, is an important enabler of low-cost mobile robot perception. Previous approaches to this problem suffer either from an overly complex inference engine or from an insufficient detection accuracy. To deal with these issues, we present SS3D, a single-stage monocular 3D object detector. The framework consists of (i) a CNN, which outputs a redundant representation of each relevant object in the image with corresponding uncertainty estimates, and (ii) a 3D bounding box optimizer. We show how modeling heteroscedastic uncertainty improves performance upon our baseline, and furthermore, how back-propagation can be done through the optimizer in order to train the pipeline end-to-end for additional accuracy. Our method achieves SOTA accuracy on monocular 3D object detection, while running at 20 fps in a straightforward implementation. We argue that the SS3D architecture provides a solid framework upon which high performing detection systems can be built, with autonomous driving being the main application in mind.

==> fig/regression/plot.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
    xlabel={$x$},
    ylabel={$y$},
    height=0.3\textwidth,
    xmin=0, xmax=5,
    ymin=-1.5, ymax=1.5,
    xtick={0,1,2,3,4,5},
    ytick={-1, 0, 1},
    legend pos=south west,
    legend cell align=left,
    legend style={font=\small},
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
    clip mode=individual,
]

\addplot[gray, only marks, mark=*, mark size=1pt]  table {fig/regression/plot.dat};
\addplot[dashed,mark=none,smooth,domain=0:5,very thick](\x,{sin(180*\x/pi)});
\addplot[mark=none,smooth,domain=0:5,very thick] (\x,{-0.18*\x*\x+0.52*\x+0.37});

\legend{Data, $y=\sin(x)$, Quadratic fit} 
 
\end{axis}
\end{tikzpicture}
